Prospects for Pulsar Studies at MeV Energies

Enabled by the Fermi Large Area Telescope, we now know young and recycled pulsars fill the gamma-ray sky, and we are beginning to understand their emission mechanism and their distribution throughout the Galaxy. However, key questions remain: Is there a large population of pulsars near the Galactic center? Why do the most energetic pulsars shine so brightly in MeV gamma rays but not always at GeV energies? What is the source and nature of the pair plasma in pulsar magnetospheres, and what role does the polar cap accelerator play? Addressing these questions calls for a sensitive, wide-field MeV telescope, which can detect the population of MeV-peaked pulsars hinted at by Fermi and hard X-ray telescopes and characterize their spectral shape and polarization.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
